Syzygies of string modules for special biserial algebras

We present discrete models of special biserial (SB) algebras and their string modules, drawing inspiration from cellular automata, and cast new light on patterns among syzygies. We explore applications of our models to open questions in homological algebra regarding certain triangulated subcategories of derived categories, with implications for the finitistic dimension conjectures. More pertinently, our models provide the inner workings for a new, original GAP package called SBStrips, written and implemented by the author. Its source code is freely available online and its documentation is included as an appendix. The package calculates syzygies of string modules (and much more besides) using specialised methods much more efficient than the general methods currently employed by the \QPA\ package.

==> Subsections/Virtual_syllables.tex <==
\subsection{Virtual syllables}

Next, we introduce some additional symbols for use within the formal calculation of the syzygy of a string module. These new symbols will be used to represent the occurrence of a pathological phenomenon within the syzygy calculation rather than representing any part of a string module. For this reason, we call these new symbols \emph{virtual syllables}.

\nlpass{Pathological syzygies} There is the short exact sequence
$\big(
\begin{tikzcd}[sep=small]
0 \ar[r]
  \& \soc P \ar[r]
    \& P \ar[r]
      \& P/\soc P\ar[r]
        \& 0
\end{tikzcd}\big)
$
for any pin module $P$, from which we easily conclude $\syzygy^1(P/\soc P) = \soc P$. %In our framework for modelling string modules and their syzygies,
This short exact sequence of such a string module $P/\soc P$ witnesses an unusual phenomenon, the details of which will be given later; namely its two boundaries interact with one another before yielding the syzygy $\soc P$.

To mark this unusual interaction in our framework we need new, special symbols. These symbols are bespoke: they only signify this specific phenomenon, and they never represent any actual part of a string module. For this reason, we will call these new symbols \emph{virtual syllables}.

\nlpass{Virtual syllables} Recall that the socle of a pin module is a simple module at some $Q$-vertex, and that $Q$-vertex will, by definition, be represented by an $\OQ$-vertex $i$ that satisfies $d_i=0$.

The \define{virtual syllables} at any such $i \in \OQ_0$ with $d_i =0$ are $(e_i,0,\pm1)=\big(\ilsyll{i}{0}{0}\big)^{\pm1}$.

\nrmks \ilitem{} Any reference to syllables excludes virtual syllables unless explicitly mentioned.

\ilitem{} It is unambiguous whether the symbol $\big( \ilsyll{\syllableplaceholder}{p}{\ep} \big)^{s}$ denotes a syllable or a virtual syllable, because $0 < \len p + \ep$ for syllables and $ 0 = \len p + \ep $ for virtual syllables.

==> contents-page.tex <==
\pagenumbering{roman}
\setcounter{page}{1}

\tableofcontents
\newpage

==> hyphenations.tex <==
% Get nice linebreaks
\hyphenation{co-loc-ali-sing}
\hyphenation{com-ple-ment}
\hyphenation{en-do-mor-phism}
\hyphenation{en-do-mor-phisms}
\hyphenation{in-jec-tive}
\hyphenation{mod-ule}
\hyphenation{mod-ules}
\hyphenation{mor-phism}
\hyphenation{mor-phisms}
\hyphenation{non-zero}
\hyphenation{over-quiv-er}
\hyphenation{pro-jec-tive}
\hyphenation{term-wise}
